What You See is What You Get: Local Labor Markets and Skill Acquisition

This paper highlights the potential for negative dynamic consequences of recent trends towards the formation of "skill-hubs". I first show evidence that skill acquisition is biased towards skills which are in demand in local labor markets. This fact along with large heterogeneity in outcomes by major and recent reductions in migration rates implies a significant potential for inefficient skill upgrading over time. To evaluate the impact of local bias in education in the context of standard models which focus on agglomeration effects, I develop a structural spatial model which includes educational investment. The model focuses on two sources of externalities: productivity through agglomeration and signaling. Both of these affect educational decisions tilting the balance of aggregate skill composition. Signaling externalities can provide a substantial wedge in the response to changes in skill demand and skill concentration with the potential for substantial welfare gains from a more equal distribution of skills.

==> mycommands.tex <==
%% ITEMIZE & ENUMERATE ENVIRONMENTS W/O BIG PARAGRAPH SKIPS
\usepackage{accents}
\setcounter{tocdepth}{2}

\newenvironment{itemize*}%
  {\begin{itemize}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{itemize}}
  
  \newenvironment{myquote}{%%
  \begin{itemize}[topsep=0pt]
  \item[]}{\end{itemize}}

\newenvironment{enumerate*}%
  {\begin{enumerate}%
    \setlength{\itemsep}{0pt}%
    \setlength{\parskip}{0pt}}%
  {\end{enumerate}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\usepackage{subcaption}

\usepackage[round]{natbib}
\bibliographystyle{aer}
\usepackage{sectsty} % For section format.
%% SECTION STUFF 
\sectionfont{\fontsize{13}{13}\selectfont}
\subsectionfont{\fontsize{11}{11}\selectfont}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\arabic{section}.\arabic{subsection}}

% USEFUL SYMBOLS
\newcommand{\br}{\mathbf{br}}
\newcommand{\betaswf}{\beta\operatorname{-SWF}}
\newcommand{\Pj}{\mathbb{P}_j}
\newcommand{\E}{\mathbb{E}}
\newcommand{\ee}{\mathcal{E}}
\newcommand{\yy}{\mathcal{Y}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\Gsp}{G^{SP}}
\newcommand{\starc}{\textbf{(*)}}
\newcommand{\myline}{\begin{center}\noindent\rule{8cm}{0.4pt}\end{center}}
\newcommand{\Var}{\mathbb{V}\text{ar}}
\newcommand{\Cov}{\text{Cov}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\ubar}[1]{\underline{#1}
\newcommand{\thetalow}{\ubar{\theta}}
\newcommand{\thetahi}{\bar{\theta}}
\newcommand{\nulow}{\ubar{\nu}}
\newcommand{\nuhi}{\bar{\nu}}
\newcommand{\ind}{\mathbf{1}}
\newcommand{\what}{\textcolor{red}{\textbf{(???)}}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\ctilde}{\tilde{c}}
\newcommand{\qwf}{q^{wf}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\qmin}{q^{\min}}
\newcommand{\qmax}{q^{\max}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\overline{q}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\qubar}{\underline{q}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\ytilde}{\tilde{y}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\renewcommand{\c}{\mathbf{c}}
\newcommand{\s}{\mathbf{s}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\ones}{\mathbf{1}}
\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\var}{\operatorname{var}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\bSigma}{\mathbf{\Sigma}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\MM}{\mathbf{M}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\Diff}{\operatorname{Diff}}
\renewcommand{\t}{\mathbf{t}}
\newcommand{\ql}{q_L}
\renewcommand{\d}{\text{d}}
\newcommand{\qh}{q_H}
\newcommand{\tl}{t_L}
\newcommand{\barcni}{\bar{c}_{-i}}
\newcommand{\cl}{c_L}
\newcommand{\cn}{c_N}
\newcommand{\bb}{\mathbf{b}}
\renewcommand{\th}{t_H}
\newcommand{\thetah}{\theta_H}
\newcommand{\C}{\mathcal{C}}
\newcommand{\thetal}{\theta_L}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\bxtilde}{\mathbf{\tilde{x}}}
\newcommand{\grad}{\nabla}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bep}{\boldsymbol{\epsilon}}
\newcommand{\mvpf}{\textsc{mvpf}}
\newcommand{\fe}{\textsc{fe}}
\newcommand{\wtp}{\textsc{wtp}}
\newcommand{\WS}{\operatorname{WS}}
\newcommand{\phat}{\hat{p}}
\newcommand{\vc}{\vec{c}}
\newcommand{\p}{\mathbf{p}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\SWF}{\operatorname{SWF}}
\newcommand{\default}{\text{default}}
\newcommand{\state}{\text{state }}




%% ENVIRONMENTS 
\newtheorem{theorem}{Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{corollary}{Corollary}
\newtheorem{result}{Result}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{example}[definition]{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{assumption}[theorem]{Assumption}
\renewenvironment{proof}[1][Proof]{\textbf{#1.} }{\ \rule{0.5em}{0.5em}}


